Why Do Open-Source LLMs Struggle with Data Analysis? A Systematic Empirical Study

Large Language Models (LLMs) hold promise in automating data analysis tasks, yet open-source models face significant limitations in these kinds of reasoning-intensive scenarios. In this work, we investigate strategies to enhance the data analysis capabilities of open-source LLMs. By curating a seed dataset of diverse, realistic scenarios, we evaluate model behavior across three core dimensions: data understanding, code generation, and strategic planning. Our analysis reveals three key findings: (1) Strategic planning quality serves as the primary determinant of model performance; (2) Interaction design and task complexity significantly influence reasoning capabilities; (3) Data quality demonstrates a greater impact than diversity in achieving optimal performance. We leverage these insights to develop a data synthesis methodology, demonstrating significant improvements in open-source LLMs' analytical reasoning capabilities. Code is available at https://github.com/zjunlp/DataMind.

==> tables/exp_complexity.tex <==
\begin{table}[!t]
\centering
\small 
\begin{tabular}{l|c|c}
\toprule
\multirow{1}{*}{\textbf{Difficulty}}  & \textbf{QRData} & \textbf{DiscoveryBench} \\
\midrule
\textit{Easy}  & 42.58 & 20.50  \\ 
\textit{Medium}   & 51.34 & 18.83 \\ 
\textit{Hard}  &  48.18 & 19.50  \\ 
\midrule
\textit{Medium} + \textit{Hard}   & 51.34  & 23.01   \\ 
\bottomrule
\end{tabular}
\caption{Analysis of Complexity characteristics using optimal turn settings (\% accuracy). 
Each difficulty level contains 733 samples.
% The Sample Number is 733.
}
\label{tab:table_complexity}
\end{table}

==> tables/exp_perf_compare_token_limit.tex <==
\begin{table*}[!t]
\centering
\small
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{Setting}} & \multicolumn{2}{c|}{\textbf{Max Token/ Turn 1024}} & \multicolumn{2}{c|}{\textbf{Max Token/ Turn 2048}} & \multicolumn{2}{c}{\textbf{Max Token/ Turn 4096}} \\
\cmidrule(lr){2-7}
 & \textbf{QRData} & \textbf{DiscoveryBench} & \textbf{QRData} & \textbf{DiscoveryBench} & \textbf{QRData} & \textbf{DiscoveryBench} \\
\midrule
\textbf{Original} & 0.4911 & 0.1883 & 0.4988 & 0.159 & 0.4842 & 0.1715 \\
\midrule
\textbf{Full} & 0.472 & 0.1674 & 0.4793 & 0.1715 & 0.4964 & 0.0962 \\
\midrule
\textbf{Summarized} &0.4939 &0.2008 & 0.4939 & 0.1715 & 0.5012 & 0.1883 \\
\bottomrule
\end{tabular}
\caption{Performance comparison of QRData and DiscoveryBench across different settings and token limits (\% accuracy).}
\label{tab:performance_comparison}
\end{table*}

==> tables/exp_turn_len.tex <==
\begin{table}[!t]
\centering
\small 
\scalebox{0.85}{ 
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Models} & \textbf{Training} & \textbf{QRData} & \textbf{DiscoveryBench} \\
\midrule
 Qwen2.5-7B-Instruct   & - &   41.38 \% &   14.23\% \\ 
 Qwen2.5-14B-Instruct  & - &   53.53 \% &  24.27\% \\
\midrule
\multicolumn{4}{c}{\textbf{Short(2-3 turns)}} \\
\midrule
Qwen2.5-7B-Instruct & LoRA & 47.93\% & 18.50\% \\
Qwen2.5-14B-Instruct & LoRA & 56.93\% & 25.10\% \\
\midrule
\multicolumn{4}{c}{\textbf{Medium(4-5 turns)}} \\
\midrule
Qwen2.5-7B-Instruct & LoRA & 50.24\% & 19.03\% \\
Qwen2.5-14B-Instruct & LoRA & 58.15\% & 26.57\% \\
\midrule
\multicolumn{4}{c}{\textbf{Long(6+ turns)}} \\
\midrule
Qwen2.5-7B-Instruct & LoRA & 47.94\% & 18.41\% \\
Qwen2.5-14B-Instruct & LoRA & 57.66\% & 25.82\% \\
\midrule
\multicolumn{4}{c}{\textbf{Mixed}} \\
\midrule
Qwen2.5-7B-Instruct & LoRA & 48.42\% & 16.74\% \\
Qwen2.5-14B-Instruct & LoRA & 53.77\% & 24.69 \% \\
\bottomrule
\end{tabular}
}
\caption{Impact of dialogue turn strategies across different Qwen model sizes and training methods (\% accuracy)}
\label{tab:phase1}
\end{table}
